Engineering Self-adaptive Authorisation Infrastructures

As organisations expand and interconnect, authorisation infrastructures become increasingly difficult to manage. Several solutions have been proposed, including self-adaptive authorisation, where the access control policies are dynamically adapted at run-time to respond to misuse and malicious behaviour. The ultimate goal of self-adaptive authorisation is to reduce human intervention, make authorisation infrastructures more responsive to malicious behaviour, and manage access control in a more cost effective way. In this paper, we scope and define the emerging area of self-adaptive authorisation by describing some of its developments, trends and challenges. For that, we start by identifying key concepts related to access control and authorisation infrastructures, and provide a brief introduction to self-adaptive software systems, which provides the foundation for investigating how self-adaptation can enable the enforcement of authorisation policies. The outcome of this study is the identification of several technical challenges related to self-adaptive authorisation, which are classified according to the different stages of a feedback control loop.

==> techniques-analyse_old.tex <==
\subsection{Analyse}
\label{sec:analysis}

The Analyse stage is made of two consecutive parts: the problem domain
analysis and the solution domain analysis.  The former analyses the
data provided by the Monitor stage in order to identify changes that
the system may have to respond to.  The latter occurs after a problem
has been identified, and is concerned with generating possible
alternative solutions that are able to handle the problem.  The
problem domain analysis can be further divided in two parts: the
identification of potential problems, and the assessment of the
identified problem in order to prioritise the mitigation.  In some
cases, a problem may be identified as sufficiently serious to be
addressed immediately.  At the other end of the spectrum, some
problems may be acknowledged, but ignored, as they are deemed not
critical enough to cause adaptation.

In the following, first, we present the challenges related to the
problem domain: anomaly detection, signature-based detection,
case-based detection, diagnosis, and normality detection.  Then, we
present those challenges related to both problem and solution domains
by clearly identifying how these are related to each of the domains:
perpetual evaluation, risk analysis, and threat management.  Finally,
we present those that are solely related to the solution domain of the
analysis: mitigation through model self-repair, and preventive
measures.

\subsubsection{Anomaly Detection}
\label{sec:eng:analysis:anomaly-detection}

\paragraph{\textbf{Challenge.}}
\marginpar{\tiny LM: is this not a superset of signature-based and
  case-based detection? It seems to me that both SB and CB are two
  different ways of detecting anomalies.}  \marginpar{\tiny RDL: point
  taken, we should provide something more general that can be
  instantiated into specific techniques.}  Anomaly detection is
related to the ability of the controller to identify any behaviour
that deviates from that which is perceived to be acceptable.  Since we
are essentially dealing with socio-technical systems for which it is
almost impossible to establish, from the outset, all their possible
behaviours, it is extremely challenging to clearly distinguish normal
from abnormal behaviour, i.e., what is acceptable and what it is not.
First, there is the uncertainty of the context of the system that
might influence whether a particular behaviour is deemed to be normal
or abnormal.  Second, there are the previously unknown or unexpected
behaviours that need to be classified according to profiles of similar
class of behaviours.  The key challenge is to be accurate when
detecting anomalies in order to reduce misclassifications.  Since
misclassifications cannot be eliminated, it is important to associate
with those classifications levels of uncertainty.  Moreover,
considering that there is no single technique that should be able to
accurately detect a wide range of anomalies, solutions supporting
anomaly detection should support diverse techniques whose outcome
should be fused in order to provide a robust evaluation of the
acceptability of the behaviour.

In order to show the complementarity of anomalous detection
techniques, after presenting the anomaly detection challenge, we
present two further specific anomaly detection challenges that should
be used in a complementary way for improving both the responsiveness
and coverage when detecting anomalies.

\paragraph{\textbf{Relevance.}}
The ability of detecting anomalies should precede the system
capability of handling insider attacks.  Since it is difficult to
accurately identify an attack, uncertainty levels should be considered
so the system can evaluate a particular detection against its context.
The objective is to reduce the number of false positives and negatives
that might have detrimental consequences upon self-adaptive
authorisation infrastructures.

\paragraph{\textbf{Example.}}
The first scenario motivates quite well the need for having accurate
detection of a misuse regarding reading and writing requests.  If a
particular abuse is not detected in time, the privacy of the couple
might be compromised.  All the other scenarios also quite motivate the
need for having an effective and efficiency means for detecting
anomalies because the failure of not detecting an abuse might
compromise the whole system.


\subsubsection{Signature-based Detection}
\label{sec:eng:analysis:signature}

\paragraph{\textbf{Challenge.}}
One way of performing problem domain analysis is to match the data
provided by the Monitor stage against signatures of known problems.  A
signature is a pattern that should be matched against the data
provided by the Monitor stage, such as, an IP address, a particular
regular expression in a log file, a URL, a version of some software,
etc.  Signature-based detection may require the matching of several
individual signatures to identify a threat.  Administrators should be
allowed to define signatures, as well as, combinations of signatures,
and associate them with threats.  Since signatures refer to precise
pieces of information, it is possible to completely automate their
recognition, and therefore the identification of threats.

\paragraph{\textbf{Relevance.}}
Signature-based detection is a common way of identifying knows
threats.  With a sufficiently expressive language to write the
signatures and their interactions, complex analysis can be performed
to discover advanced threats.  Signature-based detection is relatively
easy to automate, but the efficiency of threat detection must be
measured in terms of precision and recall.  Furthermore,
signature-based detection is best suited to detect threats that are
known and well understood in advance.

\paragraph{\textbf{Example.}}
The second scenario provides an example for a simple signature-based
detection algorithm.  In this scenario, the system detects that the
energy retailer reads the couple's energy use too often, resulting in
a potential threat to the couple's privacy.  The detection of the
energy retailer's behaviour can be implemented using signature-based
detection, where the signature of the threat is a number of
connections from the energy retailer's IP addresses that exceeds a
pre-determined threshold in a pre-determined time frame.

\subsubsection{Case-based Detection}

\paragraph{\textbf{Challenge.}}
Compared to signature-based detection, case-based detection focuses on
observing subjects' behaviours, which are harder to model, and hence,
harder to automate.  Where signature-based detection attempts to
identify well-defined actions performed by malicious subjects,
case-based detection observes the malicious behaviour of subject that
may be attempting to circumvent signature-based detection, and allows
for decisions to be made based on the subject's behaviour model.
Moreover, instead of absolute thresholds for identifying anomaly
detection, relative thresholds comparing users behaviours can be used.
Case-based detection involves recognising a behaviour that may not be
explicitly forbidden, but still suspicious, and may only be partially
automated.

\paragraph{\textbf{Relevance.}}
It may be the case that a subject will try to circumvent automated
detection.  This is where case-based detection becomes useful.  Since
signature-based detection works by using thresholds and precise
patterns of attacks, it is tempting for the attackers to try and
perform attacks that come just short of triggering signature-based
detection.  The attacker may be slowed down because of their efforts
to avoid detection, but that does not mean that the threat does not
need to be addressed.  Case-based detection is a good way to
complement signature-based detection because of its ability to detect
and act upon those types of threats.

\paragraph{\textbf{Example.}}
Since case-based detection can complement signature-based detection,
we use the same example to illustrate both approaches.  With
signature-based detection, the intrusive energy retailer was detected
when they read the couple's energy consumption more than a pre-defined
number of times during a given time frame.  One way for the energy
retailer to avoid detection by the signature-based detection system is
to stay right under the threshold.  Finding out what the threshold may
have involved getting caught once.  The case-based detection system
may be looking at the history of the read operations by the energy
retailer.  This analysis may identify that the frequency went up until
they got caught by the signature-based detection system, before
staying just under the threshold.  This may be constructed as
suspicious behaviour, especially if the retailer had previously
performed much less read operations per time period.  Similarly, the
detection of abuse could be related to a dynamic threshold instead of
a static one.  By profiling the number of times the energy retailer
reads the energy consumption within particular time intervals, these
can be compared for detecting an abuse.  An administrator may be
notified and shown a model of the retailer's behaviour to decide
whether is their can be characterised as intrusive

\subsubsection{Diagnosis}
\label{sec:eng:analysis:diagnosis}

\paragraph{\textbf{Challenge.}}
When an attack is detected, the system may try and understand the
attack, how it was performed, what damage it caused or is causing, and
which vulnerability was used to carry it out.  Diagnosing an attack
allows the system to better understand it, and therefore to make
better decisions to defend against it.

\paragraph{\textbf{Relevance.}}
Understanding an attack is key to stopping it, as well as making sure
that it does not happen again.  A self-adaptive system that can
understand where attacks come from and how they are carried out will
be more resilient than a system that can only identify them without
understanding what caused them to be successful.

\paragraph{\textbf{Example.}}
The third scenario (Section~\ref{sec:case:scenario-3}) can be handled
much better by a self-adaptive system capable of performing diagnosis
on the attack.  A system that does \emph{not} attempt to understand
the attack may stop it by modifying the user's credentials.  However,
if the attacker used a vulnerability in the system to gain the user's
credentials, they can run the attack again once the credentials have
been re-configured.  A system that would perform advanced diagnosis,
however, may be able to identify how the attacker got hold of the
credentials, and may be able to solve the root issue, or give the
administrator useful data for them to do so manually.


\subsubsection{Normality Detection}
\label{sec:eng:analysis:normality-detection}

\paragraph{\textbf{Challenge.}}
When an attack is over and a threat does not anymore pose danger, or
when a particular risk that had previously identified has been
mitigated, the system should be able to undo the measures that were
taken for protecting the system against the attack, or the likelihood
of an attack, especially if the measures taken did affect the system's
normal operation.  This should be done without exposing the system to
other attacks.

\paragraph{\textbf{Relevance.}}
Measures taken to prevent or mitigate attacks, in the context of
self-adaptive authorisation infrastructures, often take the form of
reduced capabilities for users, or more stringent, authorisation
procedures.  If the system were not able to scale back some of the
measures taken after the event that triggered them has occurred, then
the system would tend towards locking all the users out of the system.
It is therefore crucial that the system is able to always strike the
correct balance between usability and security.

\paragraph{\textbf{Example.}}
The second scenario (Section~\ref{sec:case:scenario-2}), where the
intrusive energy retailer is prevented from reading energy consumption
data if they have done it too often, requires for the counter-measure
to be eventually lifted.  This can be done after the self-adaptive
system has assessed that the energy provider's behaviour does not pose
a threat anymore.  Failure to do so would prevent the provider from
reading data that is essential to correctly billing the users, which
may have unpleasant consequences.


% \subsubsection{Model Checking}
% \label{sec:eng:analysis:model-checking}

% \marginpar{\tiny RDL: we need to discuss this. Perhaps we need to
% change the way we write this challenge.}

% \paragraph{\textbf{Challenge.}}
% Model checking techniques allow one to verify that a model satisfies
% some properties.
% If it does not, model checking techniques can point
% out the reason why some properties are not satisfied.
% Model checking
% techniques often suffer from scalability issues caused by the state
% explosion problem.

% \paragraph{\textbf{Relevance.}}
% Some attacks could be detected using a variation of model-checking
% techniques, or static analysis of models.
% The self-adaptive system
% could maintain a model representation of the monitored system and its
% environment.
% Such a model would have to satisfy certain properties
% (e.g., reachability) to be considered secure. Alternatively, the
% satisfaction of some other properties may indicate that a threat has
% been discovered.

% \paragraph{\textbf{Example.}}
% The second scenario provides a good example for analysis based on
% model checking.
% The scenario mandates that the meter usage data can
% only be collected by an authorised party, using an encrypted
% channel.
% A model could be constructed to represent the flow of the
% data from the source to the different parties that request it, the
% authentication methods used, as well as the encryption mechanisms in
% use on the links between the source and the different parties. This
% model would evolve as new parties authenticate and collect data. A
% property that the model should satisfy would be that all links must be
% encrypted.
% \marginpar{\tiny RDL:  how model checking is able to do this? I'm not sure}
% If the model checking tool determines that a link is not
% properly encrypted, then an issue has been identified, and must be
% dealt with.

\subsubsection{Perpetual Evaluation}
\label{sec:eng:analysis:perpetual-evaluation}
% \marginpar{\tiny LM: add proactive example (log checking) and leave
% both in the same subsubsection. Rewrite a bit to separate proactive
% and 'confirmation' for each paragraph} \marginpar{\tiny RDL - this
% proactive is not that clear; evaluation at the problem domain try to
% identify new vulnerabilities and attacks, and evaluation at the
% solution domain to provide assurances}

\paragraph{\textbf{Challenge.}}
When the controller is not adapting the target system, instead of
being idle, it can perform background activities for enhancing the
resilience of the system, and one of such activities is the continuous
analysis of either the problem domain or the solution domain, which is
referred to as perpetual evaluation.  \textit{Problem domain perpetual
  evaluation} refers to activity that targets the identification of
vulnerabilities and attacks.  Regarding attacks, the perpetual
evaluation should be able to anticipate attacks that will require
adaptation before they are actually deployed, for example, a denial of
service attack.  Also, another perceived role for perpetual evaluation
is to analyse on a continuous basis the system logs in order identify
potential attacks that were not previously detected.  These analyses
should run at all times, independently whether it is responding to
changes in the environment and the system.  \textit{Solution domain
  perpetual evaluation}, on the other hand, is performed for providing
assurances about the system quality of services.  Since the analysis
for the provision of assurances can be time-consuming, in order to
avoid delaying the adaptation, evaluation should be performed on
continual basis just to confirm that the system does what is suppose
to do.  Related to this challenge is the importance for the evaluation
to learn from past analysis in order to produce results faster.

\paragraph{\textbf{Relevance.}}
Perpetual evaluation can be used alongside traditional evaluation in
order to improve the coverage in detecting insider attacks, and
enhancing the provision of assurances.  This can be done either
proactively or reactively, respectively.  If insider attacks can be
predicted to occur depending on some observable pattern of behaviour,
the adaptation measure can be taken proactively.  Since the proactive
adaptation does not block any immediate response to changes, it can
relatively slow inform the adaptations that may happen in the future.
On the other hand, reactive evaluation can be run alongside a less
accurate, traditional evaluation.  While traditional evaluation can
make fast, but imperfect, decisions, the reactive evaluation can
either confirm that the adaptation satisfies the system goal, or point
to issues that may require a rollback, or further adaptation.  This is
possible because the reactive evaluation can afford to take longer to
complete, and consider more data or more stringent constraints.  This
is especially useful in scenarios where timeliness of adaptation is
important, such as the response to insider threats.

% Perpetual evaluation is very relevant to self-adaptive authorisation
% infrastructures, where a timely response to attacks is very important.
% Perpetual evaluation can help minimise the response time, as the
% ever-changing model of the system and its context is constantly
% analysed.  \marginpar{\tiny LM - think or System 1, System 2}
% \marginpar{\tiny RDL - relevance can be seen from two perspectives:
%   reactive, system adapts quickly in order to mitigate an attack, but
%   the assurances related to the adaptation are obtained after
%   adaptation is performed; proactively, anticipating potential
%   changes, the system can evaluate potential adaptations. }

\paragraph{\textbf{Example.}}
The third scenario (Section~\ref{sec:case:scenario-3}) illustrates the
advantages of perpetual evaluation.  Detecting suspicious deletions
should be done very quickly, as one would like to minimise the data
loss.  Ideally, suspicious behaviours should be detected before any
data loss happens.  However, it may not be easy to tell the difference
between legitimate and illegitimate deletion.

Proactive evaluation could monitor the system's access logs, and
compare each user's actions to their behaviour profile, and the
behaviour profile of similar users.  If a user starts acting
suspiciously, adaptation could be triggered before the users starts
deleting sensitive data.

Using reactive evaluation could allow the system to suspend a user's
permissions when suspicious activity is detected, like the deletion of
a large number of files.  This can be achieved quickly using
traditional analysis.  The reactive evaluation could then consider
more elements, such as a longer history of the user's access data, or
access data for similar users, to determine with more confidence
whether the file deletions were likely to be legitimate or not.  If
they were legitimate, a plan to reactivate the user account can be
made.  If they were not, it confirms that the decision taken by the
traditional evaluation was the right one.

\subsubsection{Risk Analysis}
\label{sec:eng:analysis:risk-analysis}

\paragraph{\textbf{Challenge.}}
Once an attack has been detected, risk analysis can help determine how
serious the attack is and what an appropriate response to the attack
should be.  In the context of the problem domain, risk analysis
strategies may consider a range of data to determine the level of risk
to be associated with a particular attack.  The type of attack is a
factor.  Other possible factors may include the strength of the attack
(e.g., the number of attackers, or the frequency of their requests),
the resource that are targeted, etc.  In the context of the solution
domain, risk can be associated with the alternative courses of action
when adaptation is required.  Factors that influence the level of risk
are related to, for example, the coverage of the evaluation or the
impact the course of action might have upon the system.

\paragraph{\textbf{Relevance.}}
Depending on the perceived risk, there are attacks that may need to be
dealt with immediately, while others may allow for a delayed response,
or no response at all, at little to no cost on the system's security.
Whether a self-adaptive authorisation infrastructure shall react to an
attack should depend on the risk associated with the attack: the
probability of an attack to be successful, and the impact the attack
might have on the system in case is not mitigated.  Regarding the
solution domain, adaptation may be expensive, whether in terms of
time, computation power, or inconvenience to legitimate users through
degradation of the service.  Therefore, a sophisticated authorisation
framework could use risk analysis to prioritise the order in which
attacks should be addressed, and when and how to deal with them.

\paragraph{\textbf{Example.}}
A combination of the second and third scenarios
(Sections~\ref{sec:case:scenario-2} and \ref{sec:case:scenario-3},
respectively) illustrate the need for risk analysis.  In the second
scenario, the system detects that the energy retailer reads data from
the meter more often than agreed.  This issue needs to be addressed,
but might not be the most critical.  The third scenario, however,
deals with the detection of data being deleted by a malicious user.
This should be stopped as soon as possible since more data will be
lost until the issue is addressed.  If issues arising from both
scenarios are detected around the same time, and if the system is only
able to deal with one issue after the other, then the data deletion
attack should be addressed before the energy provider attack.



% If the model over which the evaluation is performed includes a list
% of deleted data, then a perpetual evaluation will detect that too
% much data is being deleted as soon as the threshold is reached. If,
% however, the analysis is only run every 5 minutes, then up to 5
% minutes could pass before the attack is detected, resulting in
% potentially large amounts of data being lost.  \marginpar{\tiny RDL
% - I'm not sure about this example.}  \marginpar{\tiny LM - SYstem 1
% cuts session; System 2 checks whether the session should have been
% cut or not, and tries to learn}

\subsubsection{Threat Management}
\label{sec:eng:analysis:potential-attacks-management}

% \marginpar{\tiny LM - Vulnerability, or threat, rather than
% potential attack. It's clearer} \marginpar{\tiny RDL - true,
% otherwise we are being recursive on the argument. However, I have
% got the impression that part of the issues raised here might be
% covered in risk analysis.}
\paragraph{\textbf{Challenge.}}
Managing how to handle potential attacks is a challenge that should
influence the self-adaptation.  First, from the perspective of the
problem domain, the authorisation infrastructure should prioritise
between potential attacks, normal operation of the system, and actual
attacks.  For example, the recurrence of a perceived low risk attack
might be a symptom of a major attack.  Moreover, the contextual
information regarding other attacks that might not be directly
correlated should be an integral part of analysis of the system state
and the state of its environment.  Second, from the perspective of the
solution domain, one has to be sure that an adaptation does not
inadvertently increase the system's attack surface, or otherwise
weakens its security measures since managing potential attacks
involves modifying the structure of the system and/or its security
policies.

\paragraph{\textbf{Relevance.}}
%\marginpar{\tiny RDL - we need to look into this.}
Any perceived attack should not be considered in isolation from its
current or historical contexts, otherwise problem domain analysis
might be incomplete, thus producing outcomes that might undermine the
mitigation of these attacks.  Likewise, from the solution domain
perspective, any measure to handle the perceived attack should take
into account other measures either being processed or already
processed.  The goal is to reduce the amount of resources needed for
handling the attack, and minimise the risk of introducing new
vulnerabilities.  Moreover, considering that known vulnerabilities
might exist in the authorisation infrastructure, these should be taken
into account when analysing measures for mitigating a perceived
attack.
% By providing defence against common attacks, it reduces the risk
% placed on the system, without requiring adaptation when an attack
% actually takes place.

\paragraph{\textbf{Example.}}
\marginpar{\tiny RDL - this is not a good example - yet to be done!}
The attack in the second scenario (Section~\ref{sec:case:scenario-2}),
where the energy provider queries the energy consumption data too
often, can be avoided by defining in advance a maximum number of
queries that can be successful in a given period of time.  This
maximum number of queries can be adapted at run-time to take changes
in the system or its context into account.


\subsubsection{Mitigation through Model Self-repair}
\label{sec:eng:analysis:mitigation-repair}

\paragraph{\textbf{Challenge.}}
When a model of the system shows that an attack is likely occurring,
model repair can be used to modify the model in order to stop the
attack.  A model repair strategy must be able to not only stop the
attack, but also ensure that no other vulnerabilities arise from the
changes made to the model.  As several attacks may be detected at the
same time, the model repair approach should also be able to stop them
all.

\paragraph{\textbf{Relevance.}}
If goals can be represented as properties that the model needs to
satisfy, then a model that does not satisfy one or several of these
properties represents an infrastructure that is not aligned with the
current goals, potentially requiring adaptation.  Model repair could
modify the model so that it satisfies (or respectively, does not
satisfy) all the required properties, and hence the goals of the
system.

\paragraph{\textbf{Example.}}
The fourth scenario (Section~\ref{sec:case:scenario-4}) can be
represented as a model that represents all the sessions currently open
for each user, together with session information such as the location
where each session was opened.  A static analysis component should be
able to determine whether the model violates a property stipulating
that all active sessions opened by the same user must have been opened
in nearby locations.  For example, a user has two sessions, one opened
from the UK and the other from Japan.  The two sessions were opened
within a short time, perhaps a few minutes.  While the user may have
used anonymity measures such as a VPN or Tor to open the sessions, it
is possible that at least one of the sessions was opened using stolen
credentials.  A model repair technique would update the model in such
a way that both sessions are closed, and new sessions for the user can
only be opened from the EMS' administration console.

\subsubsection{Preventive Measures}
\label{sec:eng:analysis:preventive-measures}

\paragraph{\textbf{Challenge.}}
Preventive measures are measures taken to prevent an attack,
\emph{before} the attack happens.  In order to achieve this, the
self-adaptive authorisation infrastructure must be able to detect when
an attack is likely to occur, and be able to deploy counter-measures
ahead of time.  This can be achieved through analysis of the models of
the system and its environment, and through analysis of previous
occurrences of attacks to detect and recognise their early signs, as
well as, potential weaknesses in the system.  The difficulty is to
correctly detect an attack before it arises, and to identify the
appropriate measures that will actually prevent the attack with
minimal impact on the system's normal operations.

\paragraph{\textbf{Relevance.}}
Taking preventive measures before an attack takes place, or
immediately as an attack starts, can prevent any loss of
confidentiality, integrity or availability of the system or the data
it processes.  Compared to an approach that would only react to
attacks once they have been detected, preventive measures, if
correctly implemented, would ensure that the attack cannot cause
damage before it is detected and dealt with.

\paragraph{\textbf{Example.}}
The first scenario (Section~\ref{sec:case:scenario-1}) would benefit
from the implementation of preventive measures.  In that scenario, a
compromised service issues commands to the couple's appliances that
will increase, rather than decrease, their energy consumption.  If the
self-adaptive authorisation infrastructure can detect that the third
party service has been compromised \emph{before} the first malicious
command is issued, or at least before it is enacted, then it may be
able to revoke the service's credentials and ignore the malicious
commands, ensuring that none of them are carried out.
